The Present and Future Status of Heavy Neutral Leptons

The existence of non-zero neutrino masses points to the likely existence of multiple SM neutral fermions. When such states are heavy enough that they cannot be produced in oscillations, they are referred to as Heavy Neutral Leptons (HNLs). In this white paper we discuss the present experimental status of HNLs including colliders, beta decay, accelerators, as well as astrophysical and cosmological impacts. We discuss the importance of continuing to search for HNLs, and its potential impact on our understanding on key fundamental questions, and additionally we outline the future prospects for next-generation future experiments or upcoming accelerator run scenarios.

==> reactor.tex <==
\subsubsection{HNL searches at reactors }

In this section we discuss the opportunity for a search of HNL particles with a mass in the MeV range in short baseline reactor experiments.
Nuclear reactors are a widely used source of electron antineutrinos in the intermediate energy range up to 12 MeV. If the mixing between electron antineutrinos and a heavy neutral counterpart exist, they can produce a measurable rate of HNL in the mass range
up to 12 MeV. Up to date, no dedicated reactor experiment exists to search for HNLs in this mass range. There exists, however a sizeable variety of short and long baseline neutrino oscillation experiments worldwide, operating at various distances from either commercial nuclear power plants or research reactors. For HNL masses and couplings
relevant to the current best exclusion limits for a decay in flight measurement, the decay probability at distances ranging from meters to kilometers away from the production source can be considered as uniform. Therefore, the total detectable HNL flux for increasing reactor-detector distance can be compensated with a larger detector volume, and especially a larger solid angle coverage of the sensitive detectors. The HNL production rate will scale linearly with reactor power, together with the reactor induced gamma and/or neutron background, thus favoring experiments at high power reactors. Backgrounds can be further reduced by an appropriate detector location providing natural shielding or by the use of dedicated active or passive shielding.

In this mass range the 
 visible decay channel are HNL $\rightarrow \nu e^+e^-$ and radiative modes
 HNL $\rightarrow \nu \gamma, \nu\gamma\gamma$
 leading to two electromagnetic signature activities in the detector. 
 In the energy range of the reactor neutrinos the dominant decay into visible particles is the $e+e-$ mode. 
 A pioneering analysis in this field is reporting in~\cite{Hagner:1995bn}, reporting 
 limits down to a few times $\vert V_{eN}\vert^2 \sim 10^{-4}$ in the mass range of 2 to 7 MeV.
 In the energy range of the reactor neutrinos the dominant decay into visible particles is the $e+e-$ mode. 
 

Very short baseline neutrino experiments combine interesting features of being located at very close proximity to either power or research reactors, and capable of background reduction via pulse shape discrimination and/or segmentation. Their detection technologies are typically based on liquid and plastic/composite scintillators. 
A number of experiments is installed at a distance roughly between 
  5-25m away from intense reactor cores, at
 O(100) MW research or O(1) GW commercial reactors, and 
 with 1 to 5 m$^3$ volume detectors. These are  
 currently taking data or have recorded a large amount of data in the last few years. 
An overview of the existing and planned detectors of this type 
is given in \cite{Lasserre:2014ita}. While the design of these experiments are optimized
to address long standing reactor anomalies through the  precise measurements of the 
inverse beta decay  process, ie the measurement of of a prompt positron and a delayed thermalised neutron that is captured,
 most could also probe the decay in flight to electron positron pairs induced by HNLs without
 any specific modification to their design or operations.
 
 
The experiments often use  a trigger scheme designed to detect the captured neutron,
 which is absent in HNL decays. However, most of the short baseline detectors already
 have an electromagnetic energy threshold trigger in place, used to either calibrate or
 monitor the detector stability. Such a trigger scheme is likely suitable to detect the stopped
 electromagnetic decay products of an HNL in the mass range between 1 and 12 MeV.
 The key challenges for such a study are the control of the large anticipated backgrounds from photons of the reactor, intrinsic radioactivity in the detector muon and neutron backgrounds which need to be mastered, and depend on the detailed capabilities 
 of the experiments. 
 We believe that  there is opportunity to improve on direct experimental limits in this 
 mass range with dedicated analyses on present and possible future reactor experiments, and strongly encourage to explore that.
 
 
 
 
 
 
 
